Generative Interactions: Weaving Multiparty Human Motion with Bilevel Latent Dynamics

Human social behaviour is not a collection of independent motions, but a jointly organised process in which group dynamics and individual variation continuously shape one another. Yet existing social motion models often prioritise plausible trajectories while leaving interaction state implicit, limiting their ability to transfer across groups, tasks, and partial-observation regimes. To address this gap, we introduce Bilevel Representations for Agent Interaction Dynamics (BRAID), a hierarchical sequential latent-variable model for generative multi-person interaction. BRAID explicitly formulates social motion generation as a meta-transfer learning problem: shared interaction priors are learned across datasets and adapted through arbitrary context sets of observed people and joints. The model represents each scene through a group-level latent state that captures shared interaction dynamics and person-level latent states that capture individual behaviour conditioned on the evolving group context. This modelling choice enables coherent generation under full, sparse, or partial observations while exposing compact social-state vectors that can serve as an interface for downstream embodied-agent systems. We evaluate BRAID under a unified SMPL-based representation on social forecasting, tracking and in-filling, and response generation, using metrics that assess not only reconstruction accuracy but also realism, diversity, temporal alignment, and interpersonal coordination. We further analyse the hierarchical latent space, showing that it captures separable group- and individual-level structure.

==> figs/process_diagram_styles.tex <==
% Shared visual language for the Neural Process comparison.
\definecolor{processInk}{HTML}{384453}%
\definecolor{processLatent}{HTML}{EEE7F6}%
\definecolor{processOutput}{HTML}{E4ECF8}%
\definecolor{processContext}{HTML}{E1F1ED}%
\definecolor{processTarget}{HTML}{FAEBDD}%
\definecolor{processQuery}{HTML}{FFF0B3}%
\definecolor{processBlue}{HTML}{4169A2}%
\definecolor{processTeal}{HTML}{338D84}%
\definecolor{processOrange}{HTML}{C58043}%
\definecolor{processPurple}{HTML}{9B5E98}%
\definecolor{processGold}{HTML}{9A7100}%
\colorlet{processPanelFill}{processInk!2}%
\tikzset{%
  process node/.style={draw=processInk!75, line width=0.55pt,%
    inner sep=1pt, font=\small, text=processInk},%
  process latent/.style={process node, circle, fill=processLatent,%
    font=\footnotesize, minimum size=9.5mm},%
  process output/.style={process node, circle, fill=processOutput,%
    font=\footnotesize, minimum size=9.5mm},%
  process context/.style={process node, rounded corners=1.5pt,%
    fill=processContext, minimum width=7mm, minimum height=5.5mm},%
  process target/.style={process context, fill=processTarget},%
  process query/.style={process context, fill=processQuery, draw=processGold},%
  process edge/.style={-{Stealth[length=1.45mm,width=1.05mm]},%
    line width=0.65pt, line cap=round, line join=round,%
    shorten <=0.7pt, shorten >=0.7pt},%
  process generative/.style={process edge, draw=processBlue},%
  process temporal/.style={process edge, draw=processInk, line width=0.75pt},%
  process inference/.style={process edge, draw=processPurple,%
    dash pattern=on 2pt off 1.4pt},%
  process posterior/.style={process edge, draw=processOrange,%
    line width=0.5pt, dash pattern=on 2pt off 1.4pt},%
  process conditioning/.style={process edge, draw=processTeal, line width=0.5pt},%
  process query edge/.style={process edge, draw=processGold, line width=0.5pt},%
  process panel/.style={draw=processInk!12, fill=processPanelFill,%
    rounded corners=3pt, line width=0.4pt},%
  process label/.style={font=\footnotesize, text=processInk!85}%
}%

